EnsIR: An Ensemble Algorithm for Image Restoration via Gaussian Mixture Models

Image restoration has experienced significant advancements due to the development of deep learning. Nevertheless, it encounters challenges related to ill-posed problems, resulting in deviations between single model predictions and ground-truths. Ensemble learning, as a powerful machine learning technique, aims to address these deviations by combining the predictions of multiple base models. Most existing works adopt ensemble learning during the design of restoration models, while only limited research focuses on the inference-stage ensemble of pre-trained restoration models. Regression-based methods fail to enable efficient inference, leading researchers in academia and industry to prefer averaging as their choice for post-training ensemble. To address this, we reformulate the ensemble problem of image restoration into Gaussian mixture models (GMMs) and employ an expectation maximization (EM)-based algorithm to estimate ensemble weights for aggregating prediction candidates. We estimate the range-wise ensemble weights on a reference set and store them in a lookup table (LUT) for efficient ensemble inference on the test set. Our algorithm is model-agnostic and training-free, allowing seamless integration and enhancement of various pre-trained image restoration models. It consistently outperforms regression based methods and averaging ensemble approaches on 14 benchmarks across 3 image restoration tasks, including super-resolution, deblurring and deraining. The codes and all estimated weights have been released in Github.

==> fig/deblur_gopro_1/show_.tex <==
\begin{figure*}
\captionsetup[subfigure]{justification=centering}
  \centering
  \begin{minipage}{0.238\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim= 0 0 703 0,clip, width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_lq.png}
  \end{subfigure}
    \subcaption[]{Image}
    \end{minipage}
  \hfill
  \begin{minipage}{0.755\linewidth}
    \centering
    \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_gt.png}
    \subcaption[]{Reference \\ PSNR / SSIM}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_lq.png}
    \subcaption[]{Blurry \\ 27.352 / 0.9184}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_hist_gradient_boosting.jpg}
    \subcaption[]{Restormer~\cite{zamir2022restormer} \\ 29.980 / 0.9377}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_hist_gradient_boosting.jpg}
    \subcaption[]{HGBT~\cite{ke2017lightgbm} \\ 32.110 / 0.9481}
  \end{subfigure}
  
    \centering
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_avg.jpg}
    \subcaption[]{Average \\ 32.177 / 0.9479}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_zzpm.jpg}
    \subcaption[]{ZZPM~\cite{zhang2023ntire} \\ 32.170 / 0.9475}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_ours_64.jpg}
    \subcaption[]{Ours w/ \(b=64\) \\ 32.314 / 0.9482}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/deblur_gopro_1/deblur_GoPro_GOPR0410_11_00-000230_patch0_ours.jpg}
    \subcaption[]{Ours w/ \(b=16\) \\ 32.584 / 0.9486}
  \end{subfigure}
    \end{minipage}
  \hfill
    \vspace{-2mm}
  \caption{A visual comparison of ensemble on an image from GoPro~\cite{nah2017deep} for the task of image deblurring.
  Please zoom in for better visual quality.}
  \label{fig:deblur_gopro_1}
  \vspace{-2mm}
\end{figure*}

==> fig/dehaze_outdoor_1/show.tex <==
\begin{figure}[H]
\captionsetup[subfigure]{justification=centering}
  \centering
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim= 130 113 113 0,clip, width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_gt.png}
  \end{subfigure}
    \subcaption[]{Image}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_gt.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_lq.jpg}
  \end{subfigure}
    \subcaption[]{GT \& LQ \\ {\footnotesize PSNR / SSIM}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_MixeDehazeNet.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_erromap0_MixeDehazeNet.jpg}
  \end{subfigure}
    \subcaption[]{{\footnotesize MixDehaze} \\  {\footnotesize35.374 / 0.982}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_hist_gradient_boosting.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_erromap0_hist_gradient_boosting.jpg}
  \end{subfigure}
    \subcaption[]{HGBT {\footnotesize 34.877 / 0.984}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_avg.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_erromap0_avg.jpg}
  \end{subfigure}
    \subcaption[]{Average {\footnotesize 35.537 / 0.985}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_zzpm.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_erromap0_zzpm.jpg}
  \end{subfigure}
    \subcaption[]{ZZPM {\footnotesize 35.537 / 0.985}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_patch0_ours.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/dehaze_outdoor_1/dehaze_outdoor_0091_erromap0_ours.jpg}
  \end{subfigure}
    \subcaption[]{Ours \\ {\footnotesize 35.813 / 0.986}}
    \end{minipage}
  \hfill
    \vspace{-2mm}
  \caption{A visual comparison of ensemble on OTS for dehazing. 
  ``GT \& LQ'' means ground-truth and low quality images. 
  The second line of (c)-(g) are error maps between result and GT. ``MixDehaze'' is the abbreviation of MixDehazeNet.}
  \label{fig:dehaze_outdoor_1}
  \vspace{-3mm}
\end{figure}

==> fig/derain_test100_1/show_.tex <==
\begin{figure*}[t]
\captionsetup[subfigure]{justification=centering}
  \centering
  \begin{minipage}{0.238\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim= 0 0 0 30,clip, width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_lq.png}
  \end{subfigure}
    \subcaption[]{Image}
    \end{minipage}
  \hfill
  \begin{minipage}{0.755\linewidth}
    \centering
    \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_gt.png}
    \subcaption[]{Clean \\ PSNR / SSIM}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_lq.png}
    \subcaption[]{Rainy \\ 23.856 / 0.7682}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_MPRnet.png}
    \subcaption[]{MPRNet~\cite{zamir2021multi} \\ 34.008 / 0.9359}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_hist_gradient_boosting.jpg}
    \subcaption[]{HGBT~\cite{ke2017lightgbm} \\ 37.052 / 0.9615}
  \end{subfigure}
  
    \centering
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_avg.jpg}
    \subcaption[]{Average \\ 36.775 / 0.9603}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_zzpm.jpg}
    \subcaption[]{ZZPM~\cite{zhang2023ntire} \\ 36.777 / 0.9601}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_ours_64.jpg}
    \subcaption[]{Ours w/ \(b=64\) \\ 37.072 / 0.9618}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/derain_test100_1/derain_Test100_72_patch0_ours.jpg}
    \subcaption[]{Ours w/ \(b=32\) \\ 37.372 / 0.9639}
  \end{subfigure}
    \end{minipage}
  \hfill
    \vspace{-2mm}
  \caption{A visual comparison of ensemble on an image from Test100~\cite{zhang2019image} for the task of image deraining.
  Please zoom in for better visual quality.}
  \label{fig:derain_test100_1}
  \vspace{-3mm}
\end{figure*}

==> fig/llie_lolv1_1/show.tex <==
\begin{figure*}[htbp]
\captionsetup[subfigure]{justification=centering}
  \centering
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim= 0 0 337 0,clip, width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_gt.png}
  \end{subfigure}
    \subcaption[]{Image}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_gt.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_lq.png}
  \end{subfigure}
    \subcaption[]{GT \& LQ \\ {\footnotesize PSNR / SSIM}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_CIDNet.png}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_erromap0_CIDNet.png}
  \end{subfigure}
    \subcaption[]{CIDNet \\ {\footnotesize 25.683 / 0.915}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_hist_gradient_boosting.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_erromap0_hist_gradient_boosting.jpg}
  \end{subfigure}
    \subcaption[]{HGBT \\ {\footnotesize 26.629 / 0.888}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_avg.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_erromap0_avg.jpg}
  \end{subfigure}
    \subcaption[]{Average \\ {\footnotesize 28.889 / 0.916}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_zzpm.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_erromap0_zzpm.jpg}
  \end{subfigure}
    \subcaption[]{ZZPM \\ {\footnotesize 28.831 / 0.916}}
    \end{minipage}
  \hfill
  \begin{minipage}{0.137\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_patch0_ours.jpg}
  \end{subfigure}
  \begin{subfigure}{1\linewidth}
    \includegraphics[width=1\linewidth]{fig/llie_lolv1_1/LLIE_LOLv1_79_erromap0_ours.jpg}
  \end{subfigure}
    \subcaption[]{Ours \\ {\footnotesize 31.012 / 0.917}}
    \end{minipage}
  \hfill
    \vspace{-2mm}
  \caption{A visual comparison of ensemble on LOLv1 for low-light image enhancement. 
  ``GT \& LQ'' means ground-truth and low quality images. 
  The second line of (c)-(g) are error maps.}
  \label{fig:llie_lolv1_1}
  \vspace{-1mm}
\end{figure*}

==> fig/sr_manga109_1/show_.tex <==
\begin{figure*}
\captionsetup[subfigure]{justification=centering}
  \centering
  \begin{minipage}{0.238\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim= 0 0 0 150,clip, width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_gt.png}
  \end{subfigure}
    \subcaption[]{Image}
    \end{minipage}
  \hfill
  \begin{minipage}{0.755\linewidth}
    \centering
    \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_gt.png}
    \subcaption[]{HR \\ PSNR / SSIM}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_lq_.png}
    \subcaption[]{Bicubic \\ 23.299 / 0.8756}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_SwinIR.png}
    \subcaption[]{SwinIR~\cite{liang2021swinir} \\ 33.174 / 0.9674}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_hist_gradient_boosting.jpg}
    \subcaption[]{HGBT~\cite{ke2017lightgbm} \\ 33.919 / 0.9683}
  \end{subfigure}
  
    \centering
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_avg.jpg}
    \subcaption[]{Average \\ 33.873 / 0.9695}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_zzpm.jpg}
    \subcaption[]{ZZPM~\cite{zhang2023ntire} \\ 33.874 / 0.9694}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_ours_64.jpg}
    \subcaption[]{Ours w/ \(b=64\) \\ 33.923 / 0.9696}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_manga109_1/SR_Manga109_ShimatteIkouze_vol01_patch0_ours.jpg}
    \subcaption[]{Ours w/ \(b=32\) \\ 33.935 / 0.9696}
  \end{subfigure}
    \end{minipage}
  \hfill
    \vspace{-2mm}
  \caption{A visual comparison of ensemble on an image from Manga109~\cite{matsui2017sketch} for the task of super-resolution.
  Please zoom in for better visual quality.}
  \label{fig:sr_manga109_1}
  \vspace{-3mm}
\end{figure*}

==> fig/sr_set5_1/show.tex <==
\begin{figure*}
\captionsetup[subfigure]{justification=centering}
  \centering
  \begin{minipage}{0.238\linewidth}
    \centering
  \begin{subfigure}{1\linewidth}
    \includegraphics[trim= 0 0 0 100,clip, width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_gt.png}
  \end{subfigure}
    \subcaption[]{Image}
    \end{minipage}
  \hfill
  \begin{minipage}{0.755\linewidth}
    \centering
    \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_gt.png}
    \subcaption[]{HR \\ PSNR / SSIM}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_lq.png}
    \subcaption[]{Bicubic \\ 25.872 / 0.8861}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_SwinIR.png}
    \subcaption[]{SwinIR~\cite{liang2021swinir} \\ 31.481 / 0.9262}
  \end{subfigure}
    \centering
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_SRFormer.png}
    \subcaption[]{SRFormer~\cite{zhou2023srformer} \\ 31.588 / 0.9245}
  \end{subfigure}
    \centering
    
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_hist_gradient_boosting.jpg}
    \subcaption[]{HGBT~\cite{ke2017lightgbm} \\ 31.820 / 0.9277}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_avg.jpg}
    \subcaption[]{Average \\ 31.794 / 0.9280}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_zzpm.jpg}
    \subcaption[]{ZZPM~\cite{zhang2023ntire} \\ 31.790 / 0.9279}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.243\linewidth}
    \includegraphics[width=1\linewidth]{fig/sr_set5_1/SR_Set5_woman_patch0_ours.jpg}
    \subcaption[]{Ours w/ \(b=32\) \\ 31.835 / 0.9280}
  \end{subfigure}
    \end{minipage}
  \hfill
    % \vspace{-2mm}
  \caption{A visual comparison of ensemble on an image from Set5~\cite{bevilacqua2012low} for the task of super-resolution.
  Please zoom in for better visual quality.}
  \label{fig:sr_set5_1}
  % \vspace{-2mm}
\end{figure*}

==> sec/3_method_.tex <==
\section{Proposed Ensemble Method for Image Restoration}
\label{sec:method}

\subsection{Ensemble Formulation of Image Restoration}
Given a test set \(\mathbb{T}=\{\mathbf{\hat X}_n, \mathbf{\hat Y}_n\}\) with numerous pairs of input images and ground-truths, \(\mathbf{\hat X}_n,\mathbf{\hat Y}_n\in\mathbb{R}^{3\times H\times W}\), we have \(M\) number of pre-trained base models for image restoration, i.e., \(f_1,...,f_M: \mathbb{R}^{3\times H\times W}\rightarrow \mathbb{R}^{3\times H\times W}\).
For a model \(f_m\) where \( m\in [1,M]\), its prediction is \(\mathbf{\hat X_{m,n}} = f_m(\mathbf{\hat X}_n)\) for abbreviation. 
We consider the ensemble of the predictions as a conventional regression problem, i.e., 
%
\begin{equation}\label{eq:conventional}
    \begin{split}
        \mathbf{\tilde Y}_n = \bm{\beta}_n 
        \begin{bmatrix}
            \mathbf{\hat X_{1,n}} &\cdots & \mathbf{\hat X_{M,n}}    
        \end{bmatrix}
        ,\ \forall n
    \end{split}
\end{equation}
%
where \(\mathbf{\tilde Y}_n\) is the ensemble result, and \(\bm{\beta}_n\in \mathbb{R}^{M}\) is the vector of weight parameters for the ensemble. 
The widely used ensemble method in image restoration is averaging, where \(\bm{\beta}_n=\begin{bmatrix}
    \frac{1}{M} & \cdots & \frac{1}{M}
\end{bmatrix}\) for all samples. 
A latest method in NTIRE 2023 competition assigns the weights inversely proportional to the distance to the prediction average~\cite{zhang2023ntire}. 
RefESR~\cite{jiang2019ensemble} determines the weights based on the performances of the models on a reference set~\cite{jiang2019ensemble}. 

However, there remain several issues in their setting. 
They adopt globally constant weights for all pixels and all samples neglecting that the performances of base models may fluctuate for different patterns and samples. 
Besides, the determination of weights remains either human tuning or heavy reliance on the quality of reference set. 
Various models perform well on different data samples and thus it would be unreliable to set consistent and global weights.
% Third, as restoration models may either over-restore or under-restore different regions, it would be effective to define patch or even pixel level weights.

Alternatively, we start from the prospective of GMMs and solve the estimation of per-value weights based on EM algorithm.
The estimation is in a weak-supervised manner for better transferability to test set.

\subsection{Restoration Ensemble as Gaussian Mixture Model}

Similar to RefESR~\cite{jiang2019ensemble}, suppose we have a reference dataset \(\mathbb{D}=\{\mathbf{X}_n, \mathbf{Y}_n\}_{n=1}^N\) with \(N\) pairs of input images and ground-truths, \(\mathbf{X}_n,\mathbf{Y}_n\in\mathbb{R}^{3\times H\times W}\).
As we assume the reference set and test set follow the same data distribution, i.e., \(\mathbb{D},\mathbb{T} \sim \mathcal{D}\), such reference set would be hard to collect in real-world and thus its number \(N\) will be small.

For each model \(f_m\), its prediction is \(\mathbf{X}_{m,n} = f_m(\mathbf{X}_n)\) for abbreviation. 
We use \(\mathbf{x}_{m,n}, \mathbf{y}_n \in \mathbb{R}^L\) to represent the flattened vector of the matrices \(\mathbf{X}_{m,n}, \mathbf{Y}_n \) where \(L=3HW\). 
We can base on Gaussian prior and assume estimation error follows a zero-mean Gaussian distribution, i.e., \(\bm{\epsilon}_{m,n}=\mathbf{y}_n - \mathbf{x}_{m,n} \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}_{m,n})\) where \(\mathbf{\Sigma}_{m,n}\in \mathbb{R}^{L\times L}\) is the covariance matrix of the Gaussian. Then the observed ground-truth can be considered following the Gaussian, i.e., \(\mathbf{y}_n | f_m, \mathbf{x}_n \sim \mathcal{N}( \mathbf{x}_{m,n},\mathbf{\Sigma}_{m,n})\).
%
\begin{theorem}\label{theorem_Gaussian_add}
    Suppose \(\mathbf{X}\sim \mathcal{N}(\bm{\mu}_X, \bm{\Sigma}_X)\) and \(\mathbf{Y}\sim \mathcal{N}(\bm{\mu}_Y, \bm{\Sigma}_Y)\) are two independent random variables following multivariate Gaussian distribution. 
    If we have another random variable defined as \(\mathbf{Z}=\mathbf{X}+\mathbf{Y}\), then the variable follows \(\mathbf{Z} \sim \mathcal{N}(\bm{\mu}_X+\bm{\mu}_Y, \bm{\Sigma}_X + \bm{\Sigma}_Y) \).
\end{theorem}
%
\begin{theorem}\label{theorem_Gaussian_scalar}
    Suppose \(\mathbf{X}\sim \mathcal{N}(\bm{\mu}, \bm{\Sigma})\) is a random variable following multivariate Gaussian distribution, where \(\bm{\mu}\in \mathbb{R}^L\). 
    Given a constant vector \(\mathbf{a}\in \mathbb{R}^L\), we have the variable \(\mathbf{Y} = \mathbf{a}\cdot\mathbf{X} \sim \mathcal{N}(\mathbf{a}\cdot \bm{\mu},  \mathbf{a}^\top\mathbf{a}\cdot\bm{\Sigma}) \).
\end{theorem}
%
The proves are left in Appendix. 
As all the models are independently trained, we can assume their errors follow independent Gaussian distributions. 
Based on Theorem~\ref{theorem_Gaussian_add} and~\ref{theorem_Gaussian_scalar} , we know a weighted summation of \(\{\mathbf{y}_n | f_m, \mathbf{x}_n\}_{m=1}^M\) follows a Gaussian distribution as well.
Suppose the weight matrices of the summation are \(\bm{\alpha}_1,...,\bm{\alpha}_M\in \mathbb{R}^{L}\) such that their summation equals \(\bm{1}\).
Then we have
%
\begin{equation}
    \mathbf{y}_n | f_{1:M}, \mathbf{x}_n = \sum_{m=1}^M \bm{\alpha}_m \cdot \mathbf{y}_n | f_m, \mathbf{x}_n \sim \mathcal{N}\left(\sum_{m=1}^M \bm{\alpha}_m \cdot \mathbf{x}_{m,n} , \sum_{m=1}^M \bm{\alpha}_m^\top\bm{\alpha}_m \cdot\mathbf{\Sigma}_{m,n}\right).
\end{equation}
%
% As the weight has \(0 \le\bm{\alpha}_m\le 1\), the multi-model system enables the shrinkage of the covariance.
The ensemble result and its probability function can thus be formulated as
\begin{equation}\label{eq:gmm}
        \mathbf{\tilde y}_n = \sum_{m=1}^M \bm{\alpha}_m \cdot \mathbf{x}_{m,n};\hspace{0.5cm} 
        P(\mathbf{\tilde y}_n) =  \phi\left( \mathbf{\tilde y}_{n} \left| \sum_{m=1}^M \bm{\alpha}_m \cdot \mathbf{x}_{m,n}, \sum_{m=1}^M \bm{\alpha}_m^\top \bm{\alpha}_m \cdot\mathbf{\Sigma}_{m,n}\right.\right), 
\end{equation}
%
where \(\phi (\mathbf{y}_n|\mathbf{x}_{m,n}, \mathbf{\Sigma}_{m,n})\) is the density function of multivariate Gaussian \(\mathcal{N}(\mathbf{x}_{m,n}, \mathbf{\Sigma}_{m,n})\) and \(\mathbf{\tilde y}_n\) is the ensemble result. 
Note that Eq.~\ref{eq:conventional} forms a special case of Eq.~\ref{eq:gmm} where each weight \(\bm{\alpha}_m\) reduces to a scalar. 
The current problem of estimating \(\bm{\alpha}_m\) is still not solvable by the EM algorithm because the number of samples is \(M\) while the feature dimension is \(L\gg M\), resulting the singularity of covariance matrix when solving GMMs. 
% The model here has variate of number \(L=3H W\) but only \(M\) samples, which is hard to solve.

%
%


We thus alternatively categorize pixels into various small ranges such that the pixels within each range form a format of GMM model. 
Concretely, We separate the prediction range of models into \(T\) bins with each of width \(b\), i.e., \(\mathbb{B}=\{[0,b),[b,2b),...,[(T-1)b,255]\}\). 
The upper bound would be \(1\) instead of \(256\) if data range is within \([0,1]\).
Given a bin \(B_m=[(t-1)b,tb)\) and a pixel of prediction at location \(i\), We write an indicator function \(\mathbf{I}_{B_m}(\mathbf{x}_{m,n}^{(i)})\) such that it returns \(1\) if \(\mathbf{x}_{m,n}^{(i)} \in B_m\) and 0 otherwise.
% Thus we can categorize the prediction of a model into \(\mathbf{L}_m \in \mathbb{B}^{3\times H\times W}\). 
For the ensemble of multiple models, we traverse all possible bin sets \((B_1,\cdots,B_M)\in \mathbb{B}^M\), and define the mask map as \(\mathbf{R}_r = \prod_{m=1}^M \mathbf{I}_{B_m}(\mathbf{x}_{m,n})\in\{0,1\}^{L}\) where \(r=1,...,T^M\). 
It holds \(\sum_{r=1}^{T^M}\mathbf{R}_r = \mathbf{1}\) and \(\prod_{r=1}^{T^M}\mathbf{R}_r = \mathbf{0}\). 
For each bin set \((B_1,\cdots,B_M)\in \mathbb{B}^M\), we can select pixels of original image vectors by
%
\begin{equation}
    \mathbf{\tilde y}_{r,n} = \mathbf{R}_r \cdot \mathbf{\tilde y}_n; \hspace{1.1cm} 
    \mathbf{x}_{r,m,n} = \mathbf{R}_r \cdot \mathbf{x}_{m,n} ; \hspace{1.1cm} 
    \bm{\alpha}_{r,m} = \mathbf{R}_r \cdot \bm{\alpha}_{m} 
\end{equation}
%
The number of nonzero pixels in \(\mathbf{R}_r\) is denoted by \(N_r\). 
Thus we make a reformulation to Eq.~\ref{eq:gmm} as 
%
\begin{equation}
    \mathbf{\tilde y}_n = \sum_{r=1}^{T^M} \mathbf{\tilde y}_{r,n} = \sum_{r=1}^{T^M} \sum_{m=1}^M \mathbf{R}_r\cdot\bm{\alpha}_{r,m} \cdot \mathbf{x}_{m,n};
\end{equation}
%
\begin{theorem}\label{theorem_bonferroni}
    (Bonferroni's Inequality)
    Suppose \(X_1,..., X_n\) are \(n\) events. 
    Then we have the event \(X = \bigcap_{i=1}^n X_i\) such that the probability distribution function \(P(X) \ge \sum_i^n P(X_i) - (n-1) \) holds.
\end{theorem}
%
By Theorem~\ref{theorem_bonferroni}, we can find the lower bound of the likelihood in Eq.~\ref{eq:gmm} as 
%
\begin{equation}
\begin{split}
    & P(\mathbf{\tilde y}_n) \ge \sum_{r=1}^{T^M}  P(\mathbf{\tilde y}_{r,n}) - (T^M-1), \\
    &\text{where } P(\mathbf{\tilde y}_{r,n}) = \phi\left( \mathbf{\tilde y}_{r,n} \left| \sum_{m=1}^M \bm{\alpha}_{r,m} \cdot \mathbf{x}_{r,m,n}, \sum_{m=1}^M \bm{\alpha}_{r,m}^\top \bm{\alpha}_m \cdot\mathbf{\Sigma}_{r,m,n}\right.\right), 
\end{split}
\end{equation}
%
The equation presents the likelihood for one sample. 
We can write the maximum likelihood of estimation on the reference set by
%
\begin{equation}\label{eq:gmm_patch}
    \begin{split}
        P\left(\bigcap_{n=1}^N\mathbf{\tilde y}_{r,n}\right) \ge \sum_{n=1}^N  
        \phi\left( \mathbf{\tilde y}_{r,n} \left| \sum_{m=1}^M \bm{\alpha}_{r,m} \cdot \mathbf{x}_{r,m,n}, \sum_{m=1}^M \bm{\alpha}_{r,m}^\top \bm{\alpha}_m \cdot\mathbf{\Sigma}_{r,m,n}\right.\right) - (T^M-1) ,  
    \end{split}
\end{equation}
%



\begin{theorem}\label{theorem_boole}
    (Boole's Inequality)
    Suppose \(X_1,..., X_n\) are \(n\) events. 
    Then we have the event \(X = \bigcup_{i=1}^n X_i\) such that the probability distribution function \(P(X) \le \sum_i^n P(X_i) \) holds.
\end{theorem}

By Theorem~\ref{theorem_boole}, we have
%
\begin{equation}
        P\left(\bigcap_{n=1}^N\mathbf{\tilde y}_{r,n}\right) \ge   \phi\left( \mathbf{\tilde y}_{r,1:N} \left| \sum_{m=1}^M \bm{\alpha}_{r,m} \cdot \mathbf{x}_{r,m,1:N}, \sum_{m=1}^M \bm{\alpha}_{r,m}^\top \bm{\alpha}_m \cdot\mathbf{\Sigma}_{r,m,1:N}\right.\right) - (T^M-1),
\end{equation}

% Based on Thoerem~\ref{theorem_bonferroni}, it can be proved that the likelihood of Eq.~\ref{eq:gmm_patch} is the lower bound of Eq.~\ref{eq:gmm} (the proof is left in Appendix).
% Therefore, we can safely solve Eq.~\ref{eq:gmm_patch} alternatively.


However, we only obtain single sample for each model prediction, which hinders the optimization of the problem of finding the weights.
However, we have the observed prior knowledge of the mean of Gaussian and could help us solve the problem.

By substitution of \(\bm{\alpha}_{r,m}\) by its scalar variant \(\alpha_{r,m}\), we have
%
\begin{equation}
    \begin{split}
        P\left(\bigcap_{n=1}^N\mathbf{\tilde y}_{r,n}\right)  &\ge \frac{1}{M} \sum_{m=1}^M \alpha_{r,m} \phi\left(\mathbf{\tilde y}_{r,1:N}|\mathbf{x}_{r,m,1:N}, \mathbf{\Sigma}_{r,m,1:N}\right) \\
         &\ge \frac{1}{M} \sum_{m=1}^M \alpha_{r,m} \phi\left(\mathbf{\tilde y}_{r,1:N}|\mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N}\right),\\
         &\ge  \frac{1}{M}  \prod_{i=1}^{N_r} \sum_{m=1}^M \alpha_{r,m} \phi\left(\mathbf{\tilde y}_{r,1:N}^{(i)} \left|\mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N}\right.\right),
    \end{split}
\end{equation}
where \(\mathbf{\overline x}_{r,m,1:N} = \frac{1}{N_r} \sum_{i=1}^{N_r} \mathbf{x}^{(i)}_{r,m,1:N} \) and \(\bm{\sigma}_{r,m,1:N} = \frac{1}{N_r} \|\mathbf{x}_{r,m,1:N} - \mathbf{\overline x}_{r,m,1:N} \|_2\).

\subsection{Restoration Ensemble via Expectation Maximization}


To maximize the probability, i.e.,
%
\begin{equation}
\begin{split}
    \max \mathcal{L} &= P(\mathbf{\tilde y}_1,...,\mathbf{\tilde y}_N) \ge \sum_{m=1}^M \alpha_{r,m} \phi(\mathbf{y}_{r,1:N}|\mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N}), \\
    % &=  \sum_{n=1}^N \log \sum_{m=1}^M \alpha_m \phi(\mathbf{Y}_n|\mathbf{X}_{m,n}, \mathbf{\Sigma}_{m,n}) \\
    % &\ge \sum_{n=1}^N \log \sum_{r=1}^R \sum_{m=1}^M \alpha_{r,m} \phi(\mathbf{Y}_{r,n}|\mathbf{X}_{r,m,n}, \mathbf{\Sigma}_{r,m,n}), \\
    &\ge \sum_{m=1}^M P(z=m | \mathbf{\overline x}_{r,m,n}, \mathbf{y}_{r,1:N}, \bm{\sigma}_{r,m,1:N}) \log \frac{\alpha_{r,m} \phi(\mathbf{y}_{r,1:N} | \mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})}{P(z=m | \mathbf{\overline x}_{r,m,1:N}, \mathbf{y}_{r,1:N}, \bm{\sigma}_{r,m,1:N})} , 
\end{split}
\end{equation}

Introducing latent variable, we have

E-step:
%
\begin{equation}\label{eq:estep}
    \gamma_{r,m,1:N} \leftarrow P(z=m | \mathbf{\overline x}_{r,m,1:N}, \mathbf{y}_{r,1:N}, \bm{\sigma}_{r,m,1:N}) = \frac{\alpha_{r,m} \phi(\mathbf{y}_{r,1:N} | \mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})}{\sum_{m=1}^M \alpha_{r,m} \phi(\mathbf{y}_{r,1:N} | \mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})}
\end{equation}

M-step:
\begin{align}
    & \alpha_{r,m} \leftarrow \frac{\sum_{n}^{N_r}\gamma_{r,m,1:N}}{N_r}\label{eq:mstep-alpha} \\ 
    & \Sigma_m \leftarrow \frac{\sum_{n=1}^{N_r} \gamma_{r,m,1:N} (\mathbf{y}_{r,m,1:N} - \mu_m) (\mathbf{y}_{r,m,1:N} - \mu_m)^\top}{\sum_{n=1}^{N_r} \gamma_{r,m,1:N} } \label{eq:mstep-sigma}
\end{align}

Thanks to the separation of bins, we have the prior that
\begin{equation}
    \begin{split}
        \mu_m &\leftarrow \mathbf{\overline x}_{r,m,1:N} \\
        \Sigma_m &\leftarrow \bm{\sigma}_{r,m,1:N}
    \end{split}
\end{equation}






\input{sec/algo}

==> sec/3_method__.tex <==
\section{Proposed Ensemble Method for Image Restoration}
\label{sec:method}

In Sec.~\ref{sec:ensemble_formulation}, we first present two formulations of the ensemble problem in image restoration, i.e., global and per-pixel.
We then formulate our ensemble method in the format of Gaussian mixture models (GMMs) over partitioned per-value boxes in Sec.~\ref{sec:gmm}.
We the derive the expectation maximization (EM) algorithm with known mean and initial variance as prior knowledge to solve the GMMs problems in Sec.~\ref{sec:em}

\subsection{Ensemble Formulation of Image Restoration}\label{sec:ensemble_formulation}

Given a test set \(\mathbb{T}=\{\mathbf{\hat X}_n, \mathbf{\hat Y}_n\}\) with numerous pairs of input images and ground-truths, \(\mathbf{\hat X}_n,\mathbf{\hat Y}_n\in\mathbb{R}^{3\times H\times W}\), we have \(M\) number of pre-trained base models for image restoration, i.e., \(f_1,...,f_M: \mathbb{R}^{3\times H\times W}\rightarrow \mathbb{R}^{3\times H\times W}\).
For a model \(f_m\) where \( m\in [1,M]\), its prediction is \(\mathbf{\hat X_{m,n}} = f_m(\mathbf{\hat X}_n)\) for abbreviation. 
We consider the ensemble of the predictions as a conventional regression problem, i.e., 
%
\begin{equation}\label{eq:ensemble_global}
    \begin{split}
        \mathbf{\tilde Y}_n = \bm{\beta}_n 
        \begin{bmatrix}
            \mathbf{\hat X_{1,n}} &\cdots & \mathbf{\hat X_{M,n}}    
        \end{bmatrix}
        ,\ \forall n
    \end{split}
\end{equation}
%
where \(\mathbf{\tilde Y}_n\) is the ensemble result, and \(\bm{\beta}_n\in \mathbb{R}^{M}\) is the vector of weight parameters for the ensemble. 
The widely used ensemble method in image restoration is averaging, where \(\bm{\beta}_n=\begin{bmatrix}
    \frac{1}{M} & \cdots & \frac{1}{M}
\end{bmatrix}\) for all samples. 
A latest method in NTIRE 2023 competition assigns the weights inversely proportional to the distance to the prediction average~\cite{zhang2023ntire}. 
RefESR~\cite{jiang2019ensemble} determines the weights based on the performances of the models on a reference set~\cite{jiang2019ensemble}. 

However, there remain several issues in their setting. 
They adopt globally constant weights for all pixels and all samples neglecting that the performances of base models may fluctuate for different patterns and samples. 
Besides, the determination of weights remains either human tuning or heavy reliance on the quality of reference set. 
Various models perform well on different data samples and thus it would be unreliable to set consistent and global weights.
% Third, as restoration models may either over-restore or under-restore different regions, it would be effective to define patch or even pixel level weights.


Suppose the weight matrices of the summation are \(\bm{\alpha}_{1,n},...,\bm{\alpha}_{M,n}\in \mathbb{R}^{3\times H\times W}\) such that their summation equals \(\bm{1}\).

If we leverage regression method as ensemble approach. The formulation of pixel-wise ensemble will be 
%
\begin{equation}\label{eq:ensemble_pixel}
    \mathbf{\tilde Y}_n = \sum_{m=1}^M \bm{\alpha}_{m,n} \cdot \mathbf{X}_{m,n}
\end{equation}
%
Note that Eq.~\ref{eq:ensemble_global} forms a special case of Eq.~\ref{eq:ensemble_pixel} where each weight \(\bm{\alpha}_{m,n}\) reduces to a scalar. 

However, the formulation will result in the overfitting over reference set and the learning on outliers that are common in the case.

Alternatively, we start from the prospective of GMMs and solve the estimation of per-value weights based on EM algorithm.
The estimation is in a weak-supervised manner for better transferability to test set.

\subsection{Restoration Ensemble as Gaussian Mixture Model}\label{sec:gmm}

Similar to RefESR~\cite{jiang2019ensemble}, suppose we have a reference dataset \(\mathbb{D}=\{\mathbf{X}_n, \mathbf{Y}_n\}_{n=1}^N\) with \(N\) pairs of input images and ground-truths, \(\mathbf{X}_n,\mathbf{Y}_n\in\mathbb{R}^{3\times H\times W}\).
As we assume the reference set and test set follow the same data distribution, i.e., \(\mathbb{D},\mathbb{T} \sim \mathcal{D}\), such reference set would be hard to collect in real-world and thus its number \(N\) will be small.

For each model \(f_m\), its prediction is \(\mathbf{X}_{m,n} = f_m(\mathbf{X}_n)\) for abbreviation. 
We use \(\mathbf{x}_{m,n}, \mathbf{y}_n \in \mathbb{R}^L\) to represent the flattened vector of the matrices \(\mathbf{X}_{m,n}, \mathbf{Y}_n \) where \(L=3HW\).

We can base on Gaussian prior and assume estimation error follows a zero-mean Gaussian distribution, i.e., \(\bm{\epsilon}_{m,n}=\mathbf{y}_n - \mathbf{x}_{m,n} \sim \mathcal{N}(\mathbf{0},\mathbf{\Sigma}_{m,n})\) where \(\mathbf{\Sigma}_{m,n}\in \mathbb{R}^{L\times L}\) is the covariance matrix of the Gaussian. Then the observed ground-truth can be considered following the Gaussian, i.e., \(\mathbf{y}_n | f_m, \mathbf{x}_n \sim \mathcal{N}( \mathbf{x}_{m,n},\mathbf{\Sigma}_{m,n})\).

The reference set can then be appended as a single sample following Gaussian as
\begin{equation}
    \mathbf{y}_{1:N} | f_m, \mathbf{x}_{1:N} \sim \mathcal{N}\left( \mathbf{x}_{m,1:N},
    \diag(\mathbf{\Sigma}_{m,1},...,\mathbf{\Sigma}_{m,N})\right)
\end{equation}
%
where \(\mathbf{y}_{1:N} =\begin{bmatrix}
        \mathbf{y}_1 & \cdots & \mathbf{y}_N
    \end{bmatrix}\in\mathbb{R}^{NL}\) and \(\mathbf{x}_{m,1:N}=\begin{bmatrix}
        \mathbf{x}_{m,1} & \cdots & \mathbf{x}_{m,N}
    \end{bmatrix}\in\mathbb{R}^{NL}\) are the concatenation of observed grount-truths and flattened samples respectively, and since samples can be considered follow \textit{i.i.d} data distribution, the variance of the concatenated samples is diagonal.
%
%
% The proves are left in Appendix. 


We thus alternatively categorize pixels into various small ranges such that the pixels within each range form a format of GMM model. 
Concretely, We separate the prediction range of models into \(T\) bins with each of width \(b\), i.e., \(\mathbb{B}=\{[0,b),[b,2b),...,[(T-1)b,255]\}\). 
The upper bound would be \(1\) instead of \(256\) if data range is within \([0,1]\).
Given a bin \(B_m=[(t-1)b,tb)\) and a pixel of prediction at location \(i\), We write an indicator function \(\mathbf{I}_{B_m}(\mathbf{x}_{m,1:N}^{(i)})\) such that it returns \(1\) if \(\mathbf{x}_{m,1:N}^{(i)} \in B_m\) and 0 otherwise.
% Thus we can categorize the prediction of a model into \(\mathbf{L}_m \in \mathbb{B}^{3\times H\times W}\). 
For the ensemble of multiple models, we traverse all possible bin sets \((B_1,\cdots,B_M)\in \mathbb{B}^M\), and define the mask map as \(\mathbf{R}_r = \prod_{m=1}^M \mathbf{I}_{B_m}(\mathbf{x}_{m,1:N})\in\{0,1\}^{NL}\) where \(r=1,...,T^M\). 
It holds \(\sum_{r=1}^{T^M}\mathbf{R}_r = \mathbf{1}\) and \(\prod_{r=1}^{T^M}\mathbf{R}_r = \mathbf{0}\). 
For each bin set \((B_1,\cdots,B_M)\in \mathbb{B}^M\), we can select pixels of original image vectors by
%
\begin{equation}
    \mathbf{\tilde y}_{r,1:N} = \mathbf{R}_r \cdot \mathbf{\tilde y}_{1:N}; \hspace{1.1cm} 
    \mathbf{x}_{r,m,1:N} = \mathbf{R}_r \cdot \mathbf{x}_{m,1:N} 
\end{equation}
%

The number of nonzero pixels in \(\mathbf{R}_r\) is denoted by \(N_r\). 
Thus we make a reformulation to Eq.~\ref{eq:gmm} as 
%
\begin{equation}
    \mathbf{\tilde y}_{1:N} = \sum_{r=1}^{T^M} \mathbf{\tilde y}_{r,1:N} = \sum_{r=1}^{T^M} \sum_{m=1}^M \alpha_{r,m} \mathbf{R}_r\cdot \mathbf{x}_{m,1:N} = \sum_{r=1}^{T^M} \sum_{m=1}^M \alpha_{r,m} \cdot \mathbf{x}_{r,m,1:N} ,
\end{equation}
where \(\mathbf{\tilde y}_{1:N}=\begin{bmatrix}
        \mathbf{\tilde y}_1 & \cdots & \mathbf{\tilde y}_N
    \end{bmatrix}\in\mathbb{R}^{NL}\) denotes the concatenation of the ensemble results. 
    
% As all the models are independently trained, we can assume their errors follow independent Gaussian distributions. 
% Based on Theorem~\ref{theorem_Gaussian_add} and~\ref{theorem_Gaussian_scalar} , we know a weighted summation of \(\{\mathbf{y}_n | f_m, \mathbf{x}_n\}_{m=1}^M\) follows a Gaussian distribution as well.

% %
% \begin{equation}
%     \mathbf{y}_n | f_{1:M}, \mathbf{x}_n = \sum_{m=1}^M \bm{\alpha}_m \cdot \mathbf{y}_n | f_m, \mathbf{x}_n \sim \mathcal{N}\left(\sum_{m=1}^M \bm{\alpha}_m \cdot \mathbf{x}_{m,n} , \sum_{m=1}^M \bm{\alpha}_m^\top\bm{\alpha}_m \cdot\mathbf{\Sigma}_{m,n}\right).
% \end{equation}
% %
% As the weight has \(0 \le\bm{\alpha}_m\le 1\), the multi-model system enables the shrinkage of the covariance.


%
% where \(\phi (\mathbf{y}_n|\mathbf{x}_{m,n}, \mathbf{\Sigma}_{m,n})\) is the density function of multivariate Gaussian \(\mathcal{N}(\mathbf{x}_{m,n}, \mathbf{\Sigma}_{m,n})\) and \(\mathbf{\tilde y}_n\) is the ensemble result. 

% The current problem of estimating \(\bm{\alpha}_m\) is still not solvable by the EM algorithm because the number of samples is \(M\) while the feature dimension is \(L\gg M\), resulting the singularity of covariance matrix when solving GMMs. 
% The model here has variate of number \(L=3H W\) but only \(M\) samples, which is hard to solve.

%
%


%
\begin{theorem}\label{theorem_bonferroni}
    (Bonferroni's Inequality)
    Suppose \(X_1,..., X_n\) are \(n\) events. 
    Then we have the event \(X = \bigcap_{i=1}^n X_i\) such that the probability distribution function \(P(X) \ge \sum_i^n P(X_i) - (n-1) \) holds.
\end{theorem}
%
By Theorem~\ref{theorem_bonferroni}, we can find the lower bound of the likelihood in Eq.~\ref{eq:gmm} as 
%
\begin{equation}
\begin{split}
    & P(\mathbf{\tilde y}_{1:N}) \ge \sum_{r=1}^{T^M}  P(\mathbf{\tilde y}_{r,1:N}) - (T^M-1),
\end{split}
\end{equation}
%
Because there is no intersection between two boxes, we can safely separate the optimization over \(\mathbf{\tilde y}_n\) into \(T^M\) optimization problems over \(\mathbf{\tilde y}_{r,n}\), i.e.,
%
\begin{equation}
    \mathbf{\tilde y}_{r,1:N} = \sum_{m=1}^M \alpha_{r,m} \cdot \mathbf{x}_{r,m,1:N} ,
\end{equation}



% Based on Thoerem~\ref{theorem_bonferroni}, it can be proved that the likelihood of Eq.~\ref{eq:gmm_patch} is the lower bound of Eq.~\ref{eq:gmm} (the proof is left in Appendix).
% Therefore, we can safely solve Eq.~\ref{eq:gmm_patch} alternatively.


However, we have the observed prior knowledge of the mean of Gaussian and could help us solve the problem.

Since the pixels within the box are close with each other, we consider the pixels are sampled by a Gaussian with mean \(\mathbf{\overline x}_{r,m,1:N} = \frac{1}{N_r} \sum_{i=1}^{N_r} \mathbf{x}^{(i)}_{r,m,1:N}\), i.e., 
%
\begin{equation}
    \mathbf{\tilde y}_{r,1:N} \sim \mathcal{N}(\mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})   
\end{equation}
%
where \(\bm{\sigma}_{r,m,1:N} = \frac{1}{N_r} \|\mathbf{x}_{r,m,1:N} - \mathbf{\overline x}_{r,m,1:N} \|_2\).

Then we have

\begin{equation}
    \frac{1}{M}  \prod_{i=1}^{N_r} \sum_{m=1}^M \alpha_{r,m} \phi\left(\mathbf{\tilde y}_{r,1:N}^{(i)} \left|\mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N}\right.\right)
\end{equation}





\subsection{Restoration Ensemble via Expectation Maximization}\label{sec:em}


To maximize the probability, i.e.,
%
\begin{equation}
\begin{split}
    \max \mathcal{L} &= P(\mathbf{\tilde y}_1,...,\mathbf{\tilde y}_N) \ge \sum_{m=1}^M \alpha_{r,m} \phi(\mathbf{y}_{r,1:N}|\mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N}), \\
    % &=  \sum_{n=1}^N \log \sum_{m=1}^M \alpha_m \phi(\mathbf{Y}_n|\mathbf{X}_{m,n}, \mathbf{\Sigma}_{m,n}) \\
    % &\ge \sum_{n=1}^N \log \sum_{r=1}^R \sum_{m=1}^M \alpha_{r,m} \phi(\mathbf{Y}_{r,n}|\mathbf{X}_{r,m,n}, \mathbf{\Sigma}_{r,m,n}), \\
    &\ge \sum_{m=1}^M P(z=m | \mathbf{\overline x}_{r,m,n}, \mathbf{y}_{r,1:N}, \bm{\sigma}_{r,m,1:N}) \log \frac{\alpha_{r,m} \phi(\mathbf{y}_{r,1:N} | \mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})}{P(z=m | \mathbf{\overline x}_{r,m,1:N}, \mathbf{y}_{r,1:N}, \bm{\sigma}_{r,m,1:N})} , 
\end{split}
\end{equation}

Introducing latent variable, we have

E-step:
%
\begin{equation}\label{eq:estep}
    \gamma_{r,m,1:N} \leftarrow P(z=m | \mathbf{\overline x}_{r,m,1:N}, \mathbf{y}_{r,1:N}, \bm{\sigma}_{r,m,1:N}) = \frac{\alpha_{r,m} \phi(\mathbf{y}_{r,1:N} | \mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})}{\sum_{m=1}^M \alpha_{r,m} \phi(\mathbf{y}_{r,1:N} | \mathbf{\overline x}_{r,m,1:N}, \bm{\sigma}_{r,m,1:N})}
\end{equation}

M-step:
\begin{align}
    & \alpha_{r,m} \leftarrow \frac{\sum_{n}^{N_r}\gamma_{r,m,1:N}}{N_r}\label{eq:mstep-alpha} \\ 
    & \Sigma_m \leftarrow \frac{\sum_{n=1}^{N_r} \gamma_{r,m,1:N} (\mathbf{y}_{r,m,1:N} - \mu_m) (\mathbf{y}_{r,m,1:N} - \mu_m)^\top}{\sum_{n=1}^{N_r} \gamma_{r,m,1:N} } \label{eq:mstep-sigma}
\end{align}

Thanks to the separation of bins, we have the prior that
\begin{equation}
    \begin{split}
        \mu_m &\leftarrow \mathbf{\overline x}_{r,m,1:N} \\
        \Sigma_m &\leftarrow \bm{\sigma}_{r,m,1:N}
    \end{split}
\end{equation}






\input{sec/algo}

==> sec/7_supple_.tex <==

\newpage
\appendix


\section*{Appendix}

\section{Proof}

\setcounter{theorem}{0}


\subsection{Proof of Theorem~\ref{theorem_bonferroni}}
\begin{proof}


\begin{theorem}\label{theorem_bonferroni}
    (Bonferroni's Inequality)
    Suppose \(X_1,..., X_n\) are \(n\) events. 
    Then we have the event \(X = \bigcap\limits_{i=1}^n X_i\) such that the probability distribution function \(P(X) \ge \sum\limits_{i=1}^n P(X_i) - (n-1) \) holds.
\end{theorem}
%
By Theorem~\ref{theorem_bonferroni}, we can find the lower bound of the likelihood of \(\mathbf{y}_{1:N}\) as 
%
\begin{equation}
\begin{split}
    & P(\mathbf{y}_{1:N}) \ge \sum_{r=1}^{T^M}  P(\mathbf{y}_{r,1:N}) - (T^M-1), \\
    % &\text{where } P(\mathbf{y}_{r,1:N}) = \phi\left( \mathbf{y}_{r,1:N} \left| \sum_{m=1}^M \bm{\alpha}_{r,m} \cdot \mathbf{x}_{r,m,1:N}, \sum_{m=1}^M \bm{\alpha}_{r,m}^\top \bm{\alpha}_m \cdot\mathbf{\Sigma}_{r,m,1:N}\right.\right), 
\end{split}
\end{equation}
%
Because there is no intersection between two bin sets, we can safely separate the optimization of maximum likelihood over \(\mathbf{y}_{1:N}\) into \(T^M\) optimization problems of maximum likelihood over \(\mathbf{y}_{r,1:N}\).


We prove Bonferroni's Inequality by induction.
We first consider the case of \(n=1\), and it holds
%
\begin{equation}
    P(X) = P(X_1) - (1-1)= P(X_1).
\end{equation}
%
When \(n=2\), we first consider the De Morgan's Law,
%
\begin{equation}
    \left(\bigcap\limits_{i=1}^{k} X_i\right)^c = \bigcup\limits_{i=1}^{k} X_i^c,
\end{equation}
%
where the super-script \((\cdot)^c\) denotes the complement of an event.
We also have Boole's Inequality.
%
\begin{theorem}\label{theorem_boole}
    (Boole's Inequality)
    Suppose \(X_1,..., X_n\) are \(n\) events. 
    Then we have the event \(X = \bigcup_{i=1}^n X_i\) such that the probability distribution function \(P(X) \le \sum_i^n P(X_i) \) holds.
\end{theorem}
Based on the two properties above, we have Bonferroni's Inequality holds when \(n=2\):
%
\begin{equation}
\begin{split}
    P(X_1 \cap X_2) &= 1 - P\left((X_1 \cap X_2 )^c\right) \\
    & = 1 - P(X_1^c \cup X_2^c ) \\
    & \ge 1 - \sum_{i=1}^2 P(X_1^c) \\ 
    & = \sum_{i=1}^2 P(X_i) - 1 .
\end{split}
\end{equation}

%
When \(n = k\), suppose we have the following inequality holds
%
\begin{equation}
    P\left(\bigcap\limits_{i=1}^k X_i\right) \ge \sum_{i=1}^k P(X_i) - (k-1).
\end{equation}




We now want to prove the inequality for the case of \(n=k+1\),
%
\begin{equation}
\begin{split}
    P\left(\bigcap_{i=1}^{k+1} X_i \right) &= P\left( \left(\bigcap_{i=1}^{k} X_i \right) \cap X_{k+1} \right) \\
    & = P\left( \bigcap_{i=1}^{k} X_i \right) + P(X_{k+1}) - P\left( \left(\bigcap_{i=1}^{k} X_i \right) \cup X_{k+1} \right) \\ 
    & \ge \sum_{i=1}^k P(X_i) - (k-1) + P(X_{k+1}) - P\left( \left(\bigcap_{i=1}^{k} X_i \right) \cup X_{k+1} \right) \\
    & = \sum_{i=1}^{k+1} P(X_i) - (k-1)- P\left( \left(\bigcap_{i=1}^{k} X_i \right) \cup X_{k+1} \right) \\
    & \ge \sum_{i=1}^{k+1} P(X_i) - (k+1-1) \\
\end{split}
\end{equation}
%
Therefore, we complete the proof.
%
\end{proof}



% \subsection{Proof of Theorem~\ref{theorem_Gaussian_add}}

% To show Theorem~\ref{theorem_Gaussian_add}, we need to prove its univariate version, formulated as below:
% %
% \begin{theorem}\label{theorem_Gaussian_add_uni}
%     Suppose \({X}\sim \mathcal{N}({\mu}_X, {\sigma}_X)\) and \({Y}\sim \mathcal{N}({\mu}_Y, {\sigma}_Y)\) are two independent random variables following univariate Gaussian distribution. 
%     If we have another random variable defined as \({Z}={X}+{Y}\), then the variable follows \({Z} \sim \mathcal{N}({\mu}_X+{\mu}_Y, {\sigma}_X + {\sigma}_Y) \).
% \end{theorem}
% %
% \begin{proof}
% We have the cumulative probability function of \(Z\) as
% %
% \begin{equation}
%     F_Z(z) = P(Z\le z) = P(Y\le z - X) = \int_{-\infty}^\infty \phi\left(x|\mu_X, \sigma_X\right)  \int_{-\infty}^{z-x} \phi\left(Y|\mu_Y, \sigma_Y\right) dy dx,
% \end{equation}
% %
% where \(\phi\) denotes the probability density function of Gaussian distribution parameterized by mean and variance. 
% By taking the derivative of the equation, we have the probability density function of \(Z\) as below:
% %
% \begin{equation}
%     \frac{\partial F_Z(z)} {\partial z} = \int_{-\infty}^\infty \phi\left(x|\mu_X, \sigma_X\right) \phi\left(z-x|\mu_Y, \sigma_Y\right)  dx,
% \end{equation}
% %
% We plug the expression of Gaussian probability density function of Gaussian inside and have
% %
% \begin{equation}
% \begin{split}
%     \frac{\partial F_Z(z)} {\partial z} &= \int_{-\infty}^\infty \frac{1}{\sqrt{2\pi\sigma_X}} \exp{\left[-\frac{(x-\mu_X)^2}{2\sigma_X} \right]} \cdot \frac{1}{\sqrt{2\pi\sigma_Y}} \exp{\left[-\frac{\left(z-x-\mu_Y\right)^2}{2\sigma_Y}\right]}   dx, \\
%     &= \frac{1}{2\pi\sqrt{\sigma_X\sigma_Y}} \int_{-\infty}^\infty  \exp{\left[-\frac{\left(x-\mu_X\right)^2}{2\sigma_X} - \frac{\left(z-x-\mu_Y\right)^2}{2\sigma_Y}\right]}   dx, \\
%     % &= \frac{1}{2\pi\sigma_X\sigma_Y} \int_{-\infty}^\infty  \exp{\left\{-\frac{1}{2} \left[ \left(\frac{1}{\sigma_X^2} + \frac{1}{\sigma_Y^2}\right)x^2 + \left(\frac{2}{\sigma_Y^2}(\mu_Y - z) - \frac{2}{\sigma_X^2}\mu_X\right)x + \frac{1}{\sigma_X^2} + \frac{1}{\sigma_Y^2}(\mu_X - z)^2 \mu_X^2 \right] \right\}}   dx, \\
%     &= \frac{1}{\sqrt{2\pi} \sqrt{\sigma_X+\sigma_Y}} \exp \left[-\frac{1}{2}\frac{(z-\mu_X-\mu_Y)^2}{\sigma_X+\sigma_Y}\right] \\
%     & = \phi\left(z|\mu_X+\mu_Y, \sigma_X+\sigma_Y\right).
% \end{split}
% \end{equation}
% The probability density function of \(Z\) forms a Gaussian distribution function with mean \(\mu_X+\mu_Y\) and variance \(\sigma_X+\sigma_Y\)
% \end{proof}

% % Since we know each dimension of a multivariate Gaussian forms a univariate Gaussian, Theorem~\ref{theorem_Gaussian_add} can be trivially proved by applying Theorem~\ref{theorem_Gaussian_add_uni} for each dimension. 
% % More discussions can be found in \href{https://cs229.stanford.edu/section/more_on_gaussians.pdf}{https://cs229.stanford.edu/section/more\_on\_gaussians.pdf}.
% Since we know \(\mathbf{X}\) and \(\mathbf{Y}\) are independent, we can append them into a single multivariate Gaussian as
% %
% \begin{equation}
%     \mathbf{Z^+} \sim \mathcal{N}\left(\begin{bmatrix} \bm{\mu}_X \\ \bm{\mu}_Y \end{bmatrix}, \begin{bmatrix} \bm{\Sigma}_X & 0 \\
%     0 & \bm{\Sigma}_Y \end{bmatrix}\right),
% \end{equation}
% %
% where covariance items outside the matrix diagonal are 0 due to the independence.

% Thanks to the property that affine transformation of multivariate Gaussian forms Gaussian, i.e., 
% %
% \begin{equation}
%     \mathbf{Z} = \mathbf{B}\mathbf{Z}^+ \sim \mathcal{N} \left(\mathbf{B}\begin{bmatrix} \bm{\mu}_X \\ \bm{\mu}_Y \end{bmatrix}, \mathbf{B} \begin{bmatrix} \bm{\Sigma}_X & 0 \\
%     0 & \bm{\Sigma}_Y \end{bmatrix}\mathbf{B}^\top\right) = \mathcal{N} \left(\bm{\mu}_X + \bm{\mu}_Y, \bm{\Sigma}_X+\bm{\Sigma}_Y\right), 
% \end{equation}
% %
% where \(\mathbf{B} = \begin{bmatrix}
%         1 & 1
%     \end{bmatrix}\). 
% The proof concludes.

% \subsection{Proof of Theorem~\ref{theorem_Gaussian_scalar}}
% \begin{proof}
%     We can transform the element-wise multiplication vector \(\mathbf{a}\) into an affine transformation matrix \(\mathbf{A} = \diag (\mathbf{a} )\). 
%     Then we leverage the property that affine transformation of multivariate Gaussian forms Gaussian, i.e.,
%     \begin{equation}
%         \mathbf{a} \cdot \mathbf{X} = \mathbf{A} \mathbf{X} \sim \mathcal{N} \left( \mathbf{A}\bm{\mu}, \mathbf{A}\bm{\Sigma}\mathbf{A}^\top \right) 
%         = \mathcal{N} \left( \mathbf{a}\cdot\bm{\mu}, \mathbf{a}^\top \mathbf{a} \cdot\bm{\Sigma} \right)
%     \end{equation}
% \end{proof}

\subsection{Convergence of GMMs with prior means}


\subsection{Proof of Theorem~\ref{theorem2}}



Maximum likelihood estimation
%
\begin{equation}
\begin{split}
    f_1 &= \mathop{\arg\max}\limits_{f_1} \{\log P(\mathbf{Y}_n | f_1, \mathbf{X}_n)\} = \mathop{\arg\max}\limits_{f_1} \sum_{n=1}^N \log   \mathcal{N}(\mathbf{Y}_n | f_1(\mathbf{X}_n),\mathbf{\Sigma}_{1,n}) \\
    &= \mathop{\arg\min}\limits_{f_1} \sum_{n=1}^N \|f_1(\mathbf{X}_n) - \mathbf{Y}_n\|_2^2  
\end{split}
\end{equation}
%
\subsection{Proof of Decreasing Variance of Ensemble}

\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.

\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2024/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to automatically hide this section in the anonymized submission.
\end{ack}

\section*{References}


References follow the acknowledgments in the camera-ready paper. Use unnumbered first-level heading for
the references. Any choice of citation style is acceptable as long as you are
consistent. It is permissible to reduce the font size to \verb+small+ (9 point)
when listing the references.
Note that the Reference section does not count towards the page limit.
